ContextGPT: Infusing LLMs Knowledge into Neuro-Symbolic Activity Recognition Models

Context-aware Human Activity Recognition (HAR) is a hot research area in mobile computing, and the most effective solutions in the literature are based on supervised deep learning models. However, the actual deployment of these systems is limited by the scarcity of labeled data that is required for training. Neuro-Symbolic AI (NeSy) provides an interesting research direction to mitigate this issue, by infusing common-sense knowledge about human activities and the contexts in which they can be performed into HAR deep learning classifiers. Existing NeSy methods for context-aware HAR rely on knowledge encoded in logic-based models (e.g., ontologies) whose design, implementation, and maintenance to capture new activities and contexts require significant human engineering efforts, technical knowledge, and domain expertise. Recent works show that pre-trained Large Language Models (LLMs) effectively encode common-sense knowledge about human activities. In this work, we propose ContextGPT: a novel prompt engineering approach to retrieve from LLMs common-sense knowledge about the relationship between human activities and the context in which they are performed. Unlike ontologies, ContextGPT requires limited human effort and expertise. An extensive evaluation carried out on two public datasets shows how a NeSy model obtained by infusing common-sense knowledge from ContextGPT is effective in data scarcity scenarios, leading to similar (and sometimes better) recognition rates than logic-based approaches with a fraction of the effort.

==> sections/preliminaries.tex <==
%In this section, we formalize context-aware HAR and we formulate the NeSy Context-Aware HAR problem. 

%\subsection{Context-Aware Human Activity Recognition}
\label{sec:context-aware}

%Let $D_{u}$ be the dataset of raw sensor data collected from the mobile devices (e.g., smartphone, smartwatch) of a user $u$.
%let $D^\star = \bigcup_{u \in U}D_{u}$ be the union of the datasets of the users $U$. 
%Given a set of users $U=\{u_1, \dots, u_n\}$, 
%let $D^\star = \{D_{u_1},\dots,D_{u_n}\}$ be the set of datasets of all the users.
%Let $A= \{a_1, \dots, a_k \}$ be the set of considered activities.
%The dataset $D^\star$ is associated with a set of annotations $L$ that describes the activities performed by each user $u$. Each annotation $\lambda \in L$ is a tuple $\lambda = \langle u, a, t_s, t_e\rangle$ where $a$ is a label identifying the activity actually performed by $u$ during the time interval $[t_s, t_e]$. 
%
%Each user dataset $D_{u}$ is partitioned in a set of non-overlapping fixed-length windows $W_u = \{w_1,\dots,w_q\}$ with each window including $z$ seconds of consecutive raw sensor data of $D_u$. 

Similarly to previous works~\cite{arrotta2023neuro}, our notion of \emph{context} defines high-level situations occurring in the environment surrounding and including the user while sensor data are being acquired (e.g., \textit{it is raining}, \textit{location is a park}, \textit{current user's speed is high}). Let $C = \langle C_1, \dots, C_p \rangle$ be a set of possible contexts that are meaningful for the application domain.

%Considering the recognition of physical activities (e.g., walking, sitting on transport), 
% each window $w$ can be partitioned into $w^I$ and $w^C$. 
For each window $w$ (representing $z$ seconds of consecutive raw sensor data from the mobile/wearable devices of a specific user $u$), we derive two subsets $w^R$ and $w^C$: the former includes raw data that we consider appropriate for being directly processed by a data-driven model (e.g., inertial sensors data), while the latter involves raw sensor data that we consider useful for deriving higher-level contexts in $C$ through reasoning and/or abstraction. Note that $w^R$ and $w^C$ may have a non-empty intersection and $w^R \bigcup w^C = w$.
%These subsets may have a non-empty intersection and their union is the whole $w$.
%$w^R \bigcup w^C =w$. 
%,  is the remaining data that is probably less adequate for this purpose 
%The composition of $w^R$ and $w^C$ strictly depends on the target application, the available data, the knowledge model, and the available external services to obtain high-level context information.
%Our choice was driven by the characteristics of current context-aware datasets and the information considered by previous context-aware HAR works, and we believe that this aspect is orthogonal with respect to our contribution.
%Note that the context-aware HAR problem considers high-level context data as input and not directly raw context data. T
%Context aggregation can significantly , especially when the solution is based on data-driven approaches (e.g. neural networks). For instance, 
For instance, it may be appropriate to exclude raw GPS data from $w^R$ since it may be difficult to find robust correlations with activities capable of generalizing between different users (especially in data scarcity settings). On the other hand, raw GPS data can be included in $w^C$ to obtain high-level contexts more easily correlated with activities (e.g., semantic location).

Let $ca(w^C)$ be a \textit{Context Aggregation} function that derives all the most likely high-level contexts $C^w \subset C$ that occur in a window $w$. \textit{Context Aggregation} can be implemented using simple rules, available services, and/or context-aware middlewares~\cite{henricksen2005middleware}. For example, raw GPS coordinates can be used to derive the semantic location (e.g., at a restaurant, at a public park) by querying a dedicated web service.


\begin{definition}[Context-aware HAR]
Given a sensor data window $w$ obtained from a user $u$, the goal of \textit{context-aware Human Activity Recognition} is to provide to a tuple $\langle w^R, C^w \rangle$ the probability distribution $P = \langle p_1, \dots, p_k \rangle$, where $p_i$ is the probability that $u$ performed the activity $a_i$ in contexts $C^w$.%, with $\sum_{i=1}^{k} p_i = 1$.
\end{definition}


%\subsection{Neuro-Symbolic Context-aware HAR}
%\label{sec:neuro-symbolic}
\textit{Context-aware HAR} could be addressed by relying on machine learning models taking $\langle w^R, C^w \rangle$ as input. However, a more effective approach is to complement data-driven approaches with a knowledge model $K$ encoding relationships between activities the contexts.
%Neuro-Symbolic approaches, that are based on a combination of deep learning and knowledge-based methods.
%\hl{For instance, according to common-sense knowledge, the activity \textit{lying down} (i.e, horizontal body position) is less likely performed in outdoor locations (e.g., public park) when it is raining. 
For example, based on common-sense knowledge, people typically run outdoors in parks, on trails, or along sidewalks (preferably in dry weather) and indoors on a treadmill. Moreover, running requires the user to move at a positive speed.
%
The relationships between activities and the typical conditions in which they can be performed can be used in the HAR process to reduce the amount of labeled data required to learn them.
%without being learned from data.}

Given a knowledge model $K$ and a set of contexts $C^w$, let $CR(K,C^w)$ be a \textsc{Context Reasoning} function that outputs, for each activity $a_i$, a likelihood value $l(a_i)$ (a value between 0 and 1) of $a_i$ being consistent with the observed context $C^w$ according to the constraints in $K$.

\begin{definition}[Neuro-Symbolic Context-Aware HAR model]
A \textit{Neuro-Symbolic Context-Aware Human Activity Recognition} model combines a deep learning model $DNN$ and the context reasoning function $CR()$ to solve the context-aware HAR problem. 
\end{definition}

In the literature, several ways to build $K$ have been proposed, including ontologies modeled by domain experts using common-sense knowledge on HAR (or re-using existing ones) and considering semi-automatic approaches in charge of extracting knowledge from external sources (e.g., text, images, and videos from the web). In this work, we consider $K$ to be a pre-trained Large Language Model (LLM) implicitly encoding knowledge about activities and contexts, while $CR(K,C^w)$ is implemented by querying the LLM to determine the consistent activities based on $C^w$.


%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.5\linewidth]{imgs/problem_architecture.png}
%\caption{The neuro-symbolic context-aware HAR approach}
%\label{fig:problem}
%\end{figure}




